Symmetries and Expressive Requirements for Learning General Policies

State symmetries play an important role in planning and generalized planning. In the first case, state symmetries can be used to reduce the size of the search; in the second, to reduce the size of the training set. In the case of general planning, however, it is also critical to distinguish non-symmetric states, i.e., states that represent non-isomorphic relational structures. However, while the language of first-order logic distinguishes non-symmetric states, the languages and architectures used to represent and learn general policies do not. In particular, recent approaches for learning general policies use state features derived from description logics or learned via graph neural networks (GNNs) that are known to be limited by the expressive power of C_2, first-order logic with two variables and counting. In this work, we address the problem of detecting symmetries in planning and generalized planning and use the results to assess the expressive requirements for learning general policies over various planning domains. For this, we map planning states to plain graphs, run off-the-shelf algorithms to determine whether two states are isomorphic with respect to the goal, and run coloring algorithms to determine if C_2 features computed logically or via GNNs distinguish non-isomorphic states. Symmetry detection results in more effective learning, while the failure to detect non-symmetries prevents general policies from being learned at all in certain domains.

==> chapters/weisfeiler_leman.tex <==
\section{Logic and Weisfeiler-Leman Algorithms}

We now briefly revise notions about fragments of first-order logic, Weisfeiler-Leman
graph coloring algorithms, and some relations, as these are needed below.

\subsection{Logic Fragments}

$\FO_k$ is the fragment of first-order logic made of formulas with at most $k$
distinct variables, but where variables can be reutilized or requantified; e.g.,
$\varphi_1(x)\,{=}\,\exists y[ e(x,y) \land \exists x[ e(y,x) \land p(y) ]]$ in $\FO_2$
is true for object $u$ iff there are objects $v$ and $w$ such that $e(u,v)\land e(v,w) \land p(w)$.
Likewise, $\C_k$ is the logic $\FO_k$ extended with \emph{counting quantifiers} of the
form $\varphi_2(\bar x)=\exists^{\geq n} y[\phi(\bar x,y)]$ where $\phi$ belongs to $\C_{k-1}$.
If $\bar u$ is a $k$-tuple of objects, $\varphi_2(\bar u)$ is true in a structure $\A$
iff there are $n$ \emph{different} objects $y_1,y_2,\ldots,y_n$ such that $\phi(\bar u,y_i)$
is true in $\A$, for $1\leq i\leq n$.
$\C_k$ is more expressive than $\FO_k$ but less than (unrestricted) first-order.
The counting quantifiers restore some of the expressivity lost in $\FO_k$.

For logic $\L$ and integer $q\geq 0$, $\L^q$ consists of the formulas in $\L$
with \emph{quantifier rank} at most $q$, where the quantifier rank of a formula $\varphi$
is the maximum nesting depth of quantifiers in $\varphi$; e.g., the quantifier rank of
$\varphi_1(x)$ above is 2. %, and 1 plus the quantifier rank of $\phi$ for $\varphi_2$.
%Finally, a first-order definable state feature $\phi$ is $\L$-definable iff the sentences $\varphi_{\phi,v}$
%that characterize its values belong to $\L$.

\subsection{Weisfeiler-Leman (WL) Algorithms}

WL algorithms iteratively color the vertices of a graph, or tuples of vertices,
based on the colors of their ``neighbors,'' until a fixed point is reached.
Colors are generated with a \textsc{Relabel} function that injectively maps structures
over colors into colors.
%Within GNNs, colors are transformed into real vector embeddings, and multisets of colors are aggregated by permutation-invariant functions like max or sum.
We borrow notation and terminology from~\citeay{morris-et-al-jmlr2023} and \citeay{grohe:gnn}.

\medskip\noindent\textbf{1-Dim.\ WL (1-WL), also known as Color Refinement.}
Defined for undirected vertex colored graphs $G\,{=}\,(V,E,\lambda)$, the node coloring
$\wl_{i + 1}$ of vertex $v$ at iteration $i$ is:
\begin{displaymath}
    \wl_{i + 1}(v)\ \doteq\ \textsc{Relabel}\bigl(\bigl\langle \wl_i(v), \multiset{\wl_i(u) \mid u \in N(v)} \bigr\rangle\bigr)
\end{displaymath}
where $N(v)$ denotes the neighborhood of node $v$ in $G$, and the initial node
coloring for vertex $v$ is $\wl_0(v)=\lambda(v)$. This formulation assumes that
each vertex has a unique color determined by $\lambda$. For graphs with multiple
colors $\lambda_1,\lambda_2,...$, $\wl_0(v)=\textsc{Relabel}(\set{\lambda_i(v)\mid i=1,2,...})$.
The initial coloring $\wl_0(v)$ is referred as the \emph{atomic (isomorphism) type}
of the object $v$ in the structure $G$, denoted as $\atp(G,v)$.

\medskip\noindent\textbf{Folklore $k$-Dimensional WL ($k$-FWL).}
Also defined for undirected vertex-colored graphs $G\,{=}\,(V,E,\lambda)$ and $k\geq 2$,
it colors $k$-tuples $\bar{v} \in V^k$ as: %. The coloring $C^k_{i + 1}$ at iteration $i$ is:
\begin{displaymath}
    \fwl^k_{i+1}(\bar{v}) = \textsc{Relabel}\bigl(\bigl\langle \fwl^k_i(\bar{v}), M_i(\bar{v}) \bigr\rangle\bigr)
\end{displaymath}
where $M_i(\bar{v})$ is the multiset
\begin{displaymath}
    \multiset{\bigl(\fwl^k_i(\phi_1(\bar{v}, w)), \dots, \fwl^k_i(\phi_k(\bar{v}, w))\bigr) \mid w \in V} \,,
\end{displaymath}
and the function $\phi_j(\bar{v}, w)$ replaces the $j$-th component of the tuple $\bar{v}$
with the node $w$, and the initial color $\fwl^k_0(\bar{v})$ for tuple $\bar{v}$ is determined by its
atomic type $\atp(G,\bar{v})$. This type contains the edges among the vertices in
$\bar{v}$ and their colors; i.e., $\atp(G,\bar{v})=\atp(G,\bar{u})$ iff
the subgraphs induced by the vertices in the tuples $\bar{v}$ and $\bar{u}$, respectively, are isomorphic.

\Omit{% Not used in this paper
  \medskip\noindent\textbf{Relational $k$-Dimensional WL ($k$-RWL).}
  Defined for arbitrary relational structures $\A$ with universe $A$ and $k\geq 1$ \cite{grohe:gnn}.
  It colors $k$-tuples $\bar{v}\in A^k$ as
  \begin{displaymath}
      \rwl^k_{i+1}(\bar{v}) = \textsc{Relabel}\bigl(\bigl\langle \rwl^k_i(\bar{v}), M_i(\bar{v}) \bigr\rangle\bigr)
  \end{displaymath}
  where $M_i(\bar{v})$ is the multiset of tuples of the form
  \begin{displaymath}
    \bigl\langle \atp(\A,\bar{v}w),\bigl(\rwl^k_i(\phi_1(\bar{v}, w)), \dots, \rwl^k_i(\phi_k(\bar{v}, w))\bigr) \bigr\rangle
  \end{displaymath}
  for the objects $w$ in $A$, and where $\atp(\A,\bar{v}w)$ is the atomic type of the tuple $\bar{v}w$
  in the structure $\A$; i.e., $\atp(\A,\bar{v})=\atp(\A,\bar{u})$ iff the substructures induced by the
  objects in $\bar{v}$ and $\bar{u}$, respectively, are isomorphic.
  The initial coloring of tuple $\bar{v}$ is determined by its atomic type $\atp(\A,\bar{v})$.
}

\bigskip
For integer $k\geq 1$, $\hist^k_i(\cdot)$ denotes the multiset of colors
for the vertices of the input graph after $i$ iterations of $1$-WL, or $k$-FWL.
This multiset is called the \textbf{histogram of colors.}
Likewise, $\hist^k(\cdot)$ denotes the histogram for the \emph{fix point}
reached by 1-WL, or $k$-FWL, in the input graph.


\medskip\noindent
\alert{Mention facts: some relations between WL and logic, time to compute colorings, etc}

\Omit{% Not used in this paper
\begin{definition}
  Let us consider a relational signature (without constant symbols), and let $k\geq 1$ and $q\geq 0$
  be non-negative integers. The relation $\simeq^q_k$ over structures is
  $\A\,{\simeq^q_k}\,\B$ iff $\hist^k_q(\A)\,{=}\,\hist^k_q(\B)$.
  Likewise, the relation $\sim_k$ is $\A\,{\sim_k}\,\B$ iff $\hist^k(\A)\,{=}\,\hist^k(\B)$.
\end{definition}

The relations $\sim^q_k$ and $\sim_k$ can be used to test whether two structures satisfy the
same set of $\C^q_k$ and $\C_k$ formulas, respectively. Indeed,

\begin{theorem}[Main]
  \label{thm:main:2}
  Let $\Q$ be a class of problems over the STRIPS domain $D$, let $k\geq 1$ and $q\geq 0$ be
  non-negative integers, and let $\F$ be a pool of $\C^q_{k+1}$-definable features for $\Q$.
  If $k$ is bigger than the max arity of action schemas and predicates in $D$, then the
  relation $\sim^q_k$ over the reachable states in $\Q$ given by $s\sim^q_k t$ iff $\A^s\simeq^q_k\A^t$
  is \textbf{faithful and uniform.}
\end{theorem}
\Proof[Proof (sketch)]{
  \color{red!80!black}
  \textbf{To be finished.} But exploits the relations with logic.

  \textbf{Faithfulness.} Let $s$ and $t$ be two states such
  that $\A\simeq^q_k\B$ where $\A=\A^s$ and $\B=\A^t$.
  For any formula $\varphi(\bar x)$ in $\C^q_{k+1}$, and any $(k+1)$-tuples of objects $\bar u$ and $\bar v$
  such that $\rwl^k_q(\A,\bar u)=\rwl^k_q(\B,\bar v)$ (i.e., same color under $\A$ and $\B$),
  $\A^s\vDash\varphi(\bar u)$ iff $\A^t\vDash\varphi(\bar v)$.
  By the bound on arity, we can check preconditions and effects with formulas in $\C^q_k$.
  Hence, if $o(\bar u)$ is operator applicable in $\A$, then (since color histograms are equal) there
  is tuple $\bar v$ of objects in $\B$ such that $\rwl^k_q(\A,\bar u)=\rwl^k_q(\B,\bar v)$.
  Hence, the operator $o(\bar v)$ is applicable in $\B$ and results in a structure $\B'$ that
  is $\simeq^q_k$-equivalent to the structure $\A'$ that results of applying $o(\bar u)$ in $\A$.

  \textbf{Uniformity.} Since the features are $\C^q_k$ definable, then the truth value
  of the sentences that define the value of the features is the same for transitions
  $(s,s')\sim^q_k(t,t')$ (where this relation between pairs of states is defined analogously as before).
  Therefore, rules $C\mapsto E$ maintain their satisfiability.
  For the goal condition, notice that $\A$ is a goal state iff it satisfies the formula
  \begin{displaymath}
    \bigwedge_p \forall\bar u[ p_g(\bar u) \rightarrow p(\bar u)]
  \end{displaymath}
  where the conjunction is over all predicates, and the quantification rank of each conjunct equals
  the arity of the predicate $p$. Again, by the bound on the arities, goal condition can be tested
  with a $\C^q_k$ formula. Thus, if $\A\sim^q_k\B$, then $\A$ is a goal state iff $\B$ is a goal state.
}

The relation $\sim_k$ is important when $\F$ contains the transitive closure $p^*$ of a binary
predicate $p$, since $\A\,{\vDash}\,p^*(u,v)$ iff there is a integer $\ell$ such that $\A\,{\vDash}\,p^\ell(u,v)$,
where $p^\ell$ is the composition of $p$ with itself $\ell$ times.
As compositions can be defined using 3 variables, the predicate $p^\ell$ belongs to $\C^\ell_3$.
Hence, if $\A\,{\sim_k}\,\B$, then $\A\,{\vDash}\,p^*(u,v)$ iff there is pair $(u',v')$ in $\B$ such
that $\B\,{\vDash}\,p^*(u',v')$ and $\fwl^3(\A,(u,v))\,{=}\,\fwl^3(\B,(u',v'))$ where
$\fwl^k(\A,\tuple{v})$ is the \emph{fix-point coloring} of the tuple $\tuple{v}$ in the structure $\A$.

\begin{example}
  Let us consider the domain Blocks4ops for Blocksworld that contains 4 action schemas of arity 2,
  and where all predicates are of arity up to 2.
  Let $\Q$ be the class of instances for this domain with the goal $clear(x)$ for some block $x$.
  A generalized plan for $\Q$ can be obtained with two features: a Boolean feature $H$ that tells
  whether a block is being held, and the numerical feature $n$ that counts the number of blocks above $x$.
  The Boolean feature is $\C^1_1$ definable, and for $n$ we require the transitive closure for the
  $on$ predicate. Hence, the appropriate equivalence relation is $\simeq_3$ that is computed
  with 2-RWL until fix point.

  On the other hand, a general policy for the Gripper domain can be obtained with simple
  features that are definable in $\C^q_2$ for a small $q$. Hence, the appropriate relation
  is $\sim^q_2$ that is computed with $q$ iterations of 1-RWL. \qed
\end{example}

\begin{theorem}[Polynomial-time Testability]
  Let $k\geq 1$ and $q\geq 0$ be non-negative integers, and let $s$ and $t$ be two planning
  states over a common STRIPS domain.
  Testing $s\,{\sim_k}\,t$ and $s\,{\sim^q_k}\,t$ takes time $\O(k^2n^{k+1}\log n)$ where $n$
  is the number of objects in $s$, which equals the number of objects in $t$.
  If $s$ and $t$ have different number of objects, $s\,{\not\sim_k}\,t$ and $s\,{\not\sim^q_k}\,t$.
\end{theorem}
\Proof{
  \alert{** Don't have the exact proof. The time bound is the one for computing the fix-point coloring of $\rwl_k$
  in a graph with $n$ vertices. We need to perform only $q$ iterations without reaching the fix point.
  Don't have the time when the graph is substituted by a general relational structure
  but should be something similar, with perhaps some factor that depends on the number of relations. If such factor
  doesn't appear in the exponent, we are fine. Otherwise, the exponential term must be replaced by $n^{\O(k+1)}$ **}
}

These results imply that we can reduce a training set $\T$ using an abstraction that is
testable in polynomial time, for a fixed STRIPS domain $D$. However, we are not aware of efficient
implementation of the $k$-RWL algorithm. Interestingly, even though the best known algorithm
for testing graph isomorphism run in superpolynomial time in the worst case, it is actually
extremely efficient in practice.
We now see how to use it to implement the stronger $\iso$ relation.
}


